Flow dominance and factorization of transverse momentum correlations in Pb-Pb collisions at the LHC

We present the first measurement of the two-particle transverse momentum differential correlation function, $P_2\equiv\langle \Delta p_{\rm T} \Delta p_{\rm T} \rangle /\langle p_{\rm T} \rangle^2$, in Pb-Pb collisions at $\sqrt{s_{_{\rm NN}}} =$ 2.76 TeV. Results for $P_2$ are reported as a function of relative pseudorapidity ($\Delta \eta$) and azimuthal angle ($\Delta \varphi$) between two particles for different collision centralities. The $\Delta \phi$ dependence is found to be largely independent of $\Delta \eta$ for $|\Delta \eta| \geq$ 0.9. In 5% most central Pb-Pb collisions, the two-particle transverse momentum correlation function exhibits a clear double-hump structure around $\Delta \varphi = \pi$ (i.e., on the away side), which is not observed in number correlations in the same centrality range, and thus provides an indication of the dominance of triangular flow in this collision centrality. Fourier decompositions of $P_2$, studied as a function of collision centrality, show that correlations at $|\Delta \eta| \geq$ 0.9 can be well reproduced by a flow ansatz based on the notion that measured momentum correlations are strictly determined by the collective motion of the system.

==> bibliography.tex <==
%PRL V6

\begin{thebibliography}{99}

\bibitem{RHICqgp1} J. Adams {\it et al.} (STAR Collaboration),
  ``Experimental and theoretical challenges in the search for the
  quark gluon plasma: The STAR collaboration's critical assessment of
  the evidence from RHIC collisions,''  Nucl. Phys. {\bf{A757}} (2005)
  102-183, arXiv:nucl-ex/0501009 [nucl-ex].

\bibitem{RHICqgp2} K. Adcox {\it et al.} (PHENIX Collaboration),
  ``Formation of dense partonic matter in relativistic nucleus-nucleus
  collisions at RHIC: Experimental evolution by the PHENIX
  collaboration,'' Nucl. Phys. {\bf{A757}} (2005) 184-283,
  arXiv:nucl-ex/0410003 [nucl-ex].

\bibitem{RHICqgp3} I. Arsene {\it et al.} (BRAHMS Collaboration),
  ``Quark gluon plasma and color glass condensate at RHIC? The
  Persepective from the BRAHMS experiment,'' Nucl. Phys. {\bf{A757}}
  (2005) 1-27, arXiv:nucl-ex/0410020 [nucl-ex].

\bibitem{RHICqgp4} B. Back {\it et al.} (PHOBOS Collaboration),
  ``The PHOBOS perspective on discoveries at RHIC,''
  Nucl. Phys. {\bf{A757}} (2005) 28-101, arXiv:nucl-ex/0410022
  [nucl-ex].

\bibitem{LHCqgp1} K. Aamodt {\it et al.} (ALICE Collaboration),
  ``Charged-particle multiplicity density at mid-rapidity in central
  Pb--Pb collisions at $\sqrt{s_{_{\rm NN}}}=$ 2.76 TeV,''
  Phys. Lett. {\bf{105}} (2010) 252301, arXiv:1011:3916 [nucl-ex].

\bibitem{LHCqgp2} K. Aamodt {\it et al.} (ALICE Collaboration),
  ``Centrality dependence of charged particle multiplicity density at
  mid-rapidity in Pb--Pb collisions at $\sqrt{s_{_{\rm NN}}}=$ 2.76
  TeV,'' Phys. Lett. {\bf{106}} (2011) 032301, arXiv:1012:1657
  [nucl-ex].

\bibitem{LHCqgp2A} K. Krajczar {\it et al.} (CMS Collaboration),
  ``Charged hadron multiplicity and transverse energy densities in 
  Pb--Pb collisions from CMS,'' 
  J. Phys. G. {\bf{38}} (2011) 124041, CMS-PAS-HIN-11-003.
%% did not find an archive reference

\bibitem{LHCqgp3} K. Aamodt {\it et al.} (ALICE Collaboration),
  ``Elliptic flow of charged particle in Pb--Pb collisions at 2.76
  TeV,'' Phys. Lett. {\bf{105}} (2010) 252302, arXiv:1011:3914
  [nucl-ex].

\bibitem{LHCqgp4} K. Aamodt {\it et al.} (ALICE Collaboration),
  ``Centrality dependence of charged particle production at large
  transverse momentum in Pb--Pb collisions at $\sqrt{s_{_{\rm NN}}}=$
  2.76 TeV,'' Phys. Lett. {\bf{B720}} (2013) 52-62, arXiv:1208.2711
  [nucl-ex].

\bibitem{LHCqgp5} S. Chatrchyan {\it et al.} (CMS Collaboration),
  ``Dependence on pseudorapidity and centrality of charged hadron
  production in Pb--Pb collisions at a nucleon-nucleon center-of-mass
  energy of 2.76 TeV,'' JHEP {\bf{1108}} (2011) 141, arXiv:1107.4800
  [nucl-ex].

\bibitem{LHCqgp6} G. Aad {\it et al.} (ATLAS Collaboration),
  ``Observation of a Centrality-Dependent Dijet Asymmetry in Lead-Lead
  Collisions at $\sqrt{s_{_{\rm NN}}}=$ 2.76 TeV with ATLAS Detector
  at the LHC,'' Phys. Rev. Lett. {\bf{105}} (2010) 252303,
  arXiv:1011.6182 [nucl-ex].

%\bibitem{STAR-PRL90-082302-2003} {\bf STAR} Collaboration, C. Adler
%  {\it et al.} ``Disappearance of Back-To-Back High-$p_{\rm T}$
%  Hadron Correlations in Central Au+Au Collisions at $\sqrt{s_{_{\rm
%        NN}}}=$ 200 GeV,'' Phys. Rev. Lett. {\bf 90}, (2003) 082302.

%\cite{Heinz:2013th}
\bibitem{Heinz:2013th} 
  U.~Heinz and R.~Snellings,
  ``Collective flow and viscosity in relativistic heavy-ion collisions,''
  Ann.\ Rev.\ Nucl.\ Part.\ Sci.\  {\bf 63}  (2013) 123,
 %% doi:10.1146/annurev-nucl-102212-170540
  arXiv:1301.2826 [nucl-th].
  %%CITATION = doi:10.1146/annurev-nucl-102212-170540;%%

\bibitem{Voloshin:2002wa} 
  S.~A.~Voloshin,
  ``Anisotropic flow,''
  Nucl.\ Phys.\ A {\bf 715}, 379 (2003)
  doi:10.1016/S0375-9474(02)01450-1
  [nucl-ex/0210014].  
  
\bibitem{Molnar} 
  D.~Molnar and S.~A.~Voloshin,
  ``Elliptic flow at large transverse momenta from quark coalescence,''
  Phys.\ Rev.\ Lett.\  {\bf 91}, 092301 (2003),
%  doi:10.1103/PhysRevLett.91.092301
  arXiv:nucl-th/0302014.

\bibitem{STAR-PRC75-2007-054906} 
  B.~I.~Abelev {\it et al.} (STAR Collaboration), ``Mass, quark-number, and
  $\sqrt{s_{_{\rm NN}}}$ dependence of the second and fourth flow
  harmonics in ultra-relativistic nucleus-nucleus collisions,''
  Phys. Rev.  {\bf C75} (2007) 054906, arXiv:nucl-ex/0701010.

\bibitem{Abelev:2014pua} 
  B.~B.~Abelev {\it et al.} (ALICE Collaboration),
  ``Elliptic flow of identified hadrons in Pb-Pb collisions at $ \sqrt{s_{\mathrm{NN}}}=2.76 $ TeV,''
  JHEP {\bf 1506}   (2015) 190, 
  %doi:10.1007/JHEP06(2015)190
  arXiv:1405.4632 [nucl-ex].
  
\bibitem{janFiete}  
K. Aamodt {\it et  al.} (ALICE Collaboration),
``Evolution of the longitudinal and azimuthal structure of the near-side jet peak in Pb -- Pb collisions at $\sqrt{s_{_{\rm NN}}}=$ 2.76 TeV,''
Submitted to Phys. Rec. C (2016), arXiv:1609.06667  [nucl-ex].
  
\bibitem{ALICE-harmonic}  K. Aamodt {\it et
  al.} (ALICE Collaboration), 
  ``Harmonic decomposition of two particle angular correlations
  in Pb -- Pb collisions at $\sqrt{s_{_{\rm NN}}}=$ 2.76 TeV,''
  Phys. Lett.  {\bf B708}  (2012) 249-264,  arXiv:1109.2501 [nucl-ex].

\bibitem{CMS-harmonic} S. Chatrchyan {\it et al.} (CMS Collaboration), 
  ``Centrality dependence of dihadron correlations and azimuthal anisotropy
  harmonics in PbPb collisions at $\sqrt{s_{\rm NN}}=$ 2.76 TeV,''
  Eur. Phys. J. C  {\bf 72}  (2012), 10052,  arXiv:1201.3158 [nucl-ex] .

\bibitem{ATLAS-harmonic} G. Aad {\it et al.} (ATLAS Collaboration), 
  ``Measurement of the azimuthal anisotropy for charged particle
production in $\sqrt{s_{_{\rm NN}}}=$ 2.76 TeV Pb--Pb collisions with the
ATLAS detector,''
  Phys. Rev.  {\bf C86}  (2012) 014907,  arXiv:1203.3087 [hep-ex].

\bibitem{Voloshin:1999yf} S.~A.~Voloshin, V.~Koch, and H.~G.~Ritter,
``Event-by-event fluctuations in collective quantities,"
  Phys. Rev. {\bf C60}  (1999) 024901,
  %doi:10.1103/PhysRevC.60.024901
  	arXiv:nucl-th/9903060.

\bibitem{meanpt1} J. Adams {\it et al.} (STAR Collaboration),
``Systematic studies of the centrality and $\sqrt{{s}_{{}_{\mathit{NN}}}}$ dependence of the $dE_{T}/d\eta$ and $dN{}_{\mathrm{ch}}/d\eta$ in heavy ion collisions at midrapidity,"
%DOI:10.1103/PhysRevC.71.034908 10.1103/PhysRevC.71.049901
  Phys. Rev. {\bf C71} (2005) 064906, arXiv:nucl-ex/0409015.

\bibitem{Adamova:2008sx} D. Adamova {\it et  al.} (CERES Collaboration), 
  ``Scale-dependence of transverse momentum correlations in Pb-Au collisions at 158A GeV/c,"
  Nucl. Phys. {\bf A 811}  (2008) 179,
  %doi:10.1016/j.nuclphysa.2008.07.014
   arXiv:0803.2407[nucl-ex].

\bibitem{monica} M.~Sharma and C.~A.~Pruneau, 
``Methods for the study  of transverse momentum differential correlations,'' 
Phys. Rev. {\bf  C79} (2009) 024905,  arXiv:0810.0716 [nucl-ex].

\bibitem{Abelev:2014ckr} B.~B.~Abelev {\it et al.} (ALICE Collaboration), 
  ``Event-by-event mean $p_T$ fluctuations in pp and Pb -- Pb collisions at the LHC,"
  Eur. Phys. J. {\bf C 74} (2014) 3077, 
  %doi:10.1140/epjc/s10052-014-3077-y 
  arXiv:1407.5530 [nucl-ex].

\bibitem{Voloshin:2008dg}
  S.~A.~Voloshin, A.~M.~Poskanzer and R.~Snellings,
  ``Collective phenomena in non-central nuclear collisions,''
  in Landolt-Boernstein, {\em Relativistic Heavy Ion Physics},
  Vol. 1/23, p 5-54 (Springer-Verlag, 2010), arXiv:0809.2949 [nucl-ex].  


\bibitem{ALICE1} K.~Aamodt {\it et al.} (ALICE Collaboration), 
``ALICE: Physics Performance Report, Volume I,"
J. Phys. G: Nucl. Part. Phys. 30 (2004) 1517.

\bibitem{ALICE2} K.~Aamodt {\it et al.} (ALICE Collaboration), 
``ALICE: Physics Performance Report, Volume II," J. Phys. G:
  Nucl. Part. Phys. 32 (2006) 1295; 

\bibitem{ALICE3} K.~Aamodt {\it et al.} (ALICE Collaboration),
``The ALICE experiment at the CERN LHC," IOP, INST 3 (2008) S08002.

\bibitem{Pileup} B.~B.~Abelev {\it et al.} (ALICE Collaboration),
``Performance of the ALICE Experiment at the CERN LHC,"
Int. J. Mod. Phys. {\bf A 29}, 1430044  (2014).

\bibitem{ALICEeff} B.~B.~Abelev {\it et al.} (ALICE Collaboration),
``Multiplicity dependence of the average transverse momentum in p-p, p-Pb, and Pb-Pb collisions at the LHC,"
Phys. Lett. {\bf B 727} (2013) 371-380,  arXiv:1307.1094 [nucl-ex].

\bibitem{method_prc} S.~Ravan, P.~Pujahari, S.~Prasad, and C.~Pruneau,
``Correcting correlation function measurements,"
Phys. Rev. {\bf C89}  (2014)  024906,  arXiv:1311.3915 [nucl-ex].

\bibitem{monica_star} H.~Agakishiev {\it et al.} (STAR Collaboration), 
 ``Evolution of the differential transverse momentum correlation function with centrality in Au + Au collisions at $\sqrt{s_{NN}}$ = 200 GeV,"
  Phys. Lett. B {\bf 704} (2011) 467,  arXiv:1106.4334 [nucl-ex].

\bibitem{rhicv3_a} A. Adare {\it et al.} (PHENIX Collaboration), 
``Dihadron azimuthal correlations in Au+Au collisions at $\sqrt{s_{NN}}$ = 200 GeV,"
Phys. Rev. {\bf C78}  (2008)  014901,  arXiv:0801.4545 [nucl-ex] .

\bibitem{rhicv3_b} B.I. Abelev {\it et al.}  (STAR Collaboration), 
``Long range rapidity correlations and jet production in high energy nuclear collisions,"
Phys. Rev. {\bf C80}   (2009) 064912, arXiv:0909.0191 [nucl-ex].

\bibitem{rhicv3_c} B. Alver {\it et al.} (PHOBOS collaboration), 
``High transverse momentum triggered correlations over a large pseudorapidity acceptance in Au+Au Collisions at $\sqrt{s_{NN}}$ =200 GeV,"
Phys. Rev. Lett. {\bf 104}  (2010) 062301,  arXiv:0903.2811 [nucl-ex].

\bibitem{AlversRoland} B. Alver and G. Roland,
``Collision-geometry fluctuations and triangular flow in heavy-ion collisions,"
Phys. Rev. {\bf C81} (2010) 054905, arXiv:1003.0194 [nucl-th].


\bibitem{ALICE-PRL2011} K. Aamodt {\it et al.} (ALICE Collaboration), 
  ``Higher Harmonic Anisotropic Flow Measurements of Charged Particles in Pb--Pb collisions at $\sqrt{s_{_{\rm NN}}}=$ 2.76  TeV,'' Phys. Rev. Lett. {\bf 107}   (2011) 032301,  arXiv:1105.3865 [nucl-ex].


\end{thebibliography}


%% \bibitem{H-Zhang-PRL98-2007-212301} H. Zhang {\it et al.} ``Dihadron
%%   Tomography of High-Energy Nuclear Collisions in Next-to-Leading
%%   Order Perturbative QCD,'' Phys. Rev. Lett. {\bf 98} (2007) 212301.

%% \bibitem{Adler:2002pu} {\bf STAR} Collaboration, C. Adler {\it et
%%   al.} ``Elliptic flow from two and four particle correlations in
%%   Au+Au collisions at $\sqrt{s_{_{\rm NN}}}=$ 130 GeV,''
%%   Phys. Rev. {\bf C66}, 034904 (2002). [nucl-ex/0206001].


%% \bibitem{Sorensen:2009cz} P.~Sorensen, arXiv:0905.0174 [nucl-ex].

%% \bibitem{Sorensen:2006nw} {\bf STAR} Collaboration, ``Elliptic flow
%%   fluctuations in Au+Au collisions $\sqrt{s_{_{\rm NN}}}=$ 200 GeV,''
%%   J. Phys. G {\bf G34}, S897 (2007). [nucl-ex/0612021].

%% \bibitem{PHOBOS-harmonic} {\bf PHOBOS} Collaboration, B. Alver {\it et
%%   al.} Phys. Rev. {\bf C81}, 034915 (2010).

%% \bibitem{CMS-harmonic} {\bf CMS} Collaboration, S. Chatrchyan {\it et
%%   al.} Eur. Phys. J. {\bf C 72}, 2012 (2012).

%% \bibitem{ATLAS-harmonic} {\bf ATLAS} Collaboration, G. Aad {\it et
%%   al.} Phys. Rev. {\bf C 86}, 014907 (2012).





%  \bibitem{Ollit} J. Y. Ollitrault,
%  \Phys. Rev. {\bf D 46}, 229 (1992).

%  \\bibitem{Sergei-ptcor} S.~A.~Voloshin, ``Transverse radial expansion
%  \%  \  in nuclear collisions and two particle correlations,''
%  \  Phys. Lett. {\bf B632}, 490-494 (2006).

%  \\bibitem{Sergei-ptcor1} S.~A.~Voloshin, V.~Koch, and H.~G.~Ritter,
%  \  Phys. Rev. {\bf C60}, 024901 (1999)
%  \  doi:10.1103/PhysRevC.60.024901[nucl-th/9903060].
%  \

%  \\bibitem{meanpt2} {\bf STAR} Collaboration, C. Adler {\it et al.},
%  \  Phys. Rev. Lett. {\bf 90}, 172301, 2003

%  \\bibitem{meanpt3} {\bf ALICE} Collaboration, B. Abelev {\it et al.},
%  \  Eur. Phys. J. {\bf C 74}, 3077, 2014



